Practical Solutions for Machine Learning Safety in Autonomous Vehicles

Autonomous vehicles rely on machine learning to solve challenging tasks in perception and motion planning. However, automotive software safety standards have not fully evolved to address the challenges of machine learning safety such as interpretability, verification, and performance limitations. In this paper, we review and organize practical machine learning safety techniques that can complement engineering safety for machine learning based software in autonomous vehicles. Our organization maps safety strategies to state-of-the-art machine learning techniques in order to enhance dependability and safety of machine learning algorithms. We also discuss security limitations and user experience aspects of machine learning components in autonomous vehicles.

==> sections/8_VasuInputs.tex <==
\section{To be merged}


In this paper, we focus on \TODO{quantify work ahead}.

==> tables/table.tex <==
% Link to tables: https://docs.google.com/spreadsheets/d/1Pwk9q_53aGGFcegfdIwpQPPdddBJpPdNPYO1gqs2800/edit#gid=0


\begin{table*}[]
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\centering
\caption{Comparison between safety standards gaps for ML components and fundamental safety limitations of ML algorithms. \TODO{better caption}}
\label{tab:my-table}
\begin{tabular}{ccc}
\hline
\textbf{\begin{tabular}[c]{@{}c@{}}Gaps in Safety Standards \\ for ML Components\end{tabular}} & \textbf{Fundamental ML Safety Limitations} & \textbf{\begin{tabular}[c]{@{}c@{}}Machine Learning and \\ Software Safety Research\end{tabular}} \\ \hline
\multirow{2}{*}{Code Review} & Not code-based & ([ref]) \\ \cline{2-3} 
 & Not specifiable & ([ref]) \\ \hline
Software Safety Requirements Specification & Data-driven model training & ([ref]) \\ \hline
Software Architectural Design & Not code-based & ([ref]) \\ \hline
Software Unit Design & Non-converx optimization & ([ref]) \\ \hline
\multirow{2}{*}{Unit, Integration and System Testing} & Not Verifiable & ([ref]) \\
 & Non-deterministic & ([ref]) \\ \hline
Traceability & Not Transparent ([ref]) & ([ref]) \\ \hline
\end{tabular}
\end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[]
% \centering
% \caption{Algorithm dependability methods to complement functional safety and SOTIF safety methods for machine learning safety.}
% \label{tab:my-table}
% \begin{tabular}{ccc}
% \hline
% \begin{tabular}[c]{@{}c@{}}Gaps in Safety Standards \\ for ML Components\end{tabular} & Fundamental ML Safety Limitations & Machine Learning Dependability Method \\ \hline
% \multirow{2}{*}{Code Review} & Not specifiable & [ref] ...[ref] \\ \cline{2-3} 
%  & Non-deterministic & ...[ref] ...[ref] \\ \hline
% Software Safety Requirements Specification & xxxx & yyy: [ref] xxx [ref] \\ \hline 
% Software Architectural Design & xxxx & yyy: [ref] xxx [ref] \\ \hline
% Software Unit Design & Non-converx optimization & Dataset analysis: [ref] Regularization [ref] \\ \hline
% Unit, Integration and System Testing & Not Verifiable & Uncertainty Extraction: XX [ref] \\ \hline
% \multicolumn{1}{|c|}{Traceability} & Not Transparent & ... [ref] \\ \hline
% \end{tabular}
% \end{table*}



% \begin{table*}[]
% \centering
% \caption{Algorithm dependability methods to complement functional safety and SOTIF safety methods for machine learning safety.}
% \label{tab:my-table}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{@{}cccc@{}}
% \toprule
%  & ISO Software Safety Clause/Term & DNN Safety Limitations & Machine Learning Dependability Method \\ \midrule
% \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\rotatebox{90}{Functional Safety} \end{tabular}} \multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}\rotatebox{90}{(ISO 26262-6)} \end{tabular}} 
% & \multirow{2}{*}{Software Requirements Specification} & Not specifiable & Run-time Outlier Detection: ...[ref] ...[ref] \\ \cmidrule(l){3-4} 
%  &  & Non-deterministic & ...[ref] ...[ref] \\ \cmidrule(l){2-4} 
%  & Software Unit Design & Non-converx optimization & Dataset analysis: [ref] Regularization: ref] \\ \cmidrule(l){2-4} 
%  & \multirow{2}{*}{Software Unit Verification} & Not Verifiable & Uncertainty Extraction: XX [ref] \\ \cmidrule(l){3-4} 
%  &  & Not Transparent & ... [ref] \\ \midrule
% \multirow{3}{*}{\rotatebox{90}{SOTIF}} & Functional modifications to reduce SOTIF Related Risks & Robustness & ...[ref] [ref] \\ \cmidrule(l){2-4} 
%  & Verification for known-unface Scenarios &  & ...[ref] [ref] \\ \cmidrule(l){2-4} 
%  & Validation of Unknown-Unsafe Scenarios &  & ... [ref] [ref] \\ \bottomrule
% \end{tabular}%
% }
% \end{table*}
